IGANN Sparse: Bridging Sparsity and Interpretability with Non-linear Insight

Feature selection is a critical component in predictive analytics that significantly affects the prediction accuracy and interpretability of models. Intrinsic methods for feature selection are built directly into model learning, providing a fast and attractive option for large amounts of data. Machine learning algorithms, such as penalized regression models (e.g., lasso) are the most common choice when it comes to in-built feature selection. However, they fail to capture non-linear relationships, which ultimately affects their ability to predict outcomes in intricate datasets. In this paper, we propose IGANN Sparse, a novel machine learning model from the family of generalized additive models, which promotes sparsity through a non-linear feature selection process during training. This ensures interpretability through improved model sparsity without sacrificing predictive performance. Moreover, IGANN Sparse serves as an exploratory tool for information systems researchers to unveil important non-linear relationships in domains that are characterized by complex patterns. Our ongoing research is directed at a thorough evaluation of the IGANN Sparse model, including user studies that allow to assess how well users of the model can benefit from the reduced number of features. This will allow for a deeper understanding of the interactions between linear vs. non-linear modeling, number of selected features, and predictive performance.

==> acronyms.tex <==
\newacronym{pbpm}{PBPM}{predictive business process monitoring}
\newacronym{bpm}{BPM}{business process management}
\newacronym{dsr}{DSR}{design science research}
\newacronym{dnn}{DNN}{deep neural network}
\newacronym{lstm}{LSTM}{long short-term memory}
\newacronym{bilstm}{BiLSTM}{bi-directional long short-term memory}
\newacronym{ml}{ML}{machine learning}
\newacronym{dl}{DL}{deep learning}
\newacronym{pm}{PM}{process mining}
\newacronym{it}{IT}{information technology}
\newacronym{is}{IS}{information systems}
\newacronym{pdp}{PDP}{partial dependence plots}
\newacronym{ebm}{EBM}{explainable boosting machine}
\newacronym{gbm}{GBM}{gradient boosting machine}

\newacronym{xai}{XAI}{explainable artificial intelligence}
\newacronym{shap}{SHAP}{Shapley additive explanations}
\newacronym{lime}{LIME}{local interpretable model-agnostic explanations}
\newacronym{gam}{GAM}{generalized additive model}
\newacronym{gaim}{GAIM}{generalized additive index model}
\newacronym{nam}{NAM}{neural additive model}
\newacronym{xnn}{xNN}{explainable neural network}
\newacronym{exnn}{ExNN}{enhanced explainable neural network}
\newacronym{ppr}{PPR}{projection pursuit regression}
\newacronym{gaminet}{GAMI-Net}{GAMI-Net}
\newacronym{igann}{I-GANN}{interpretable generalized additive neural network}
\newacronym{vi}{VI}{variable importance}
\newacronym{ice}{ICE}{individual conditional expectation}
\newacronym{rf}{RF}{random forest}
\newacronym{dt}{DT}{decision tree}
\newacronym{svm}{SVM}{support vector machine}
\newacronym{lr}{LR}{logistic/linear regression}
\newacronym{xgb}{XGB}{extreme gradient boosting}
\newacronym{mlp}{MLP}{multi-layer perceptron}

\newacronym{rmse}{RMSE}{root mean square error}
\newacronym{mae}{MAE}{mean absolute error}
